Efficient PDE constrained shape optimization based on Steklov-Poincar\'e type metrics

Recent progress in PDE constrained optimization on shape manifolds is based on the Hadamard form of shape derivatives, i.e., in the form of integrals at the boundary of the shape under investigation, as well as on intrinsic shape metrics. From a numerical point of view, domain integral forms of shape derivatives seem promising, which rather require an outer metric on the domain surrounding the shape boundary. This paper tries to harmonize both points of view by employing a Steklov-Poincar\'e type intrinsic metric, which is derived from an outer metric. Based on this metric, efficient shape optimization algorithms are proposed, which also reduce the analytical labor, so far involved in the derivation of shape derivatives.

==> quasinewton.tex <==
\section{A quasi-Newton approach on shape manifolds}\label{quasi}
As pointed out in \cite{VHS-shape-Riemann}, shape optimization can be viewed as optimization on Riemannian shape manifolds and resulting optimization methods can be constructed and analyzed within this framework, which combines algorithmic ideas from \cite{Absil-book-2008} with the differential geometric point of view established in \cite{MM-2006}.
As in \cite{VHS-shape-Riemann}, we study connected and compact subsets $\Omega_2$ of $\R^2$ with $\Omega_2\neq\emptyset$ and $C^\infty$ boundary $\partial\Omega_2$ (cf. figure \ref{fig_Omega}).
We now identify the variable boundary $\partial \Omega_2 = \Gi$ with a simple closed curve $c\colon S^1 \to \mathbbm{R}^2$.
Additionally, we need to describe a space including all feasible shapes $\Gi$ and the corresponding tangent spaces.
In \cite{MM-2006}, this set of smooth boundary curves $c$ is characterized by  
\[
B_e(S^1,\R^2):=\mbox{Emb}(S^1,\R^2)/\mbox{Diff}(S^1)
\] 
i.e., as the set of all equivalence classes of $C^\infty$ embeddings of $S^1$ into the plane ($\mbox{Emb}(S^1,\R^2)$), where the equivalence relation is defined by the set of all $C^\infty$ re-parameterizations, i.e., diffeomorphisms of $S^1$ into itself ($\mbox{Diff}(S^1)$). A particular point on the manifold $B_e(S^1,\R^2)$ is represented by a curve $c:S^1\ni\theta\mapsto c(\theta)\in\R^2$. Because of the equivalence relation ($\mbox{Diff}(S^1)$), the tangent space is isomorphic to the set of all normal $C^\infty$ vector fields along $c$, i.e.
\[
T_cB_e\cong\{h\ |\ h=\alpha n,\, \alpha\in C^\infty(S^1,\R)\}
\]
where $n$ is the unit exterior normal field of the shape $\Omega_2$ defined by the boundary $\partial\Omega_2=c$ such that $n (\theta)\perp c^\prime$ for all $\theta\in S^1$ and $c^\prime$ denotes the circumferential derivative as in \cite{MM-2006}. For our discussion, we pick among the other metrics discussed in \cite{MM-2006} the Sobolev metric family for
$A\ge 0$
\begin{align*}
g^1:\ &T_cB_e\times T_cB_e\to \R\\
    & (h,k)\mapsto
    \int\limits_{c=\partial\Omega_2}\alpha\beta+A\alpha^\prime\beta^\prime
    ds =((id-A\triangle_c)\alpha,\beta)_{L^2(c)}
\end{align*}
where $h=\alpha n$ and $k=\beta n$ denote two elements from
the tangent space at $c$ and $\triangle_c$ denotes the Laplace-Beltrami operator on the surface $c$.  In \cite{MM-2006} it is shown that for $A>0$ the scalar product $g^1$ defines a Riemannian metric on $B_e$ and 
thus, geodesics can be used to measure distances.
Unfortunately, this is not the case for the most simple member $g^0$ of the metric family $g^1$, where $A=0$.

With the shape space $B_e$ and its tangent space in hand we can now form the Riemannian shape gradient corresponding to a shape derivative given in the form
\[
dJ[V]=\int_c \gamma\scp{V,n}ds.
\]
In our setting the shape derivative is given in theorem \ref{theorem_sg_bb} and the Riemannian metric by $g^1$.
Finally, the Riemannian shape gradient $\text{grad}J$ is obtained by
\[
\grad J=gn\, \quad \mbox{with } (id -A\triangle_c)\tilde{\gamma}=\gamma\, .
\]

In the sequel, we will also need the concept of the covariant derivative $\nabla$ and of the exponential map
\begin{align*}
\exp_c:\ &T_cB_e\to B_e\\
    & h\mapsto \exp_c(h)
\end{align*}
defining a local diffeomorphism between the tangent space and the manifold by following the locally uniquely defined geodesic starting in $c\in B_e$ with velocity $h\in T_cB_e$. The exponential map depends on the Riemannian metric $g^1$ in the usual way. 

The application of quasi-Newton methods is based on the secant condition, which is formulated on the Riemannian manifold $B_e$ analogously to  \cite{Absil-book-2008} for a step $c_{j+1}:=R_{c_j}(\eta)$ resulting from an increment $\eta_j\in T_{c_j}B_e$ in iteration $j$ via a retraction $R$ as
\[
\grad J (c_{j+1})-{\cal T}_{\eta_{j}}\grad J (c_{j})=G_{j+1}[{\cal T}_{\eta_{j}}\eta_{j}]
\]
where ${\cal T}:TB_e\oplus TB_e\to TB_e: (h_c,k_c)\mapsto {\cal T}_{h_c}k_c$ is a vector transport associated to the retraction $R$ and $G_{j+1}$ is intended to approximate the
Riemannian Hessian $\nabla\grad J(c_{j+1})$. In order to formulate the BFGS-update in a concise way, we need to introduce the following notation for a typical linear operator associated with the Riemannian metric
\begin{align*}
h\otimes k:\ &T_cB_e\to T_cB_e\\
    & v\mapsto g^1(k,v)h
\end{align*}
with this notation and together with the following abbreviations
\begin{align*}
s_j:=&{\cal T}_{\eta_{j}}\eta_{j}\in T_{c_{j+1}}B_e\\
y_j:=& \grad J (c_{j+1})-{\cal T}_{\eta_{j}}\grad J (c_{j})\in T_{c_{j+1}}B_e
\end{align*}
we can rephrase the BFGS-update on Riemannian shape space endowed with the metric $g^1$ as
\[
G_{j+1}=\tilde{G}_j-\frac{(\tilde{G}_js_j)\otimes(\tilde{G}_js_j)}{g^1(s_j,\tilde{G}_js_j)}+\frac{y_j\otimes y_j}{g^1(s_j,y_j)}
\]
where $\tilde{G}_j:={\cal T}_{\eta_j}\circ G_j\circ {\cal
  T}_{\eta_j}^{-1}$. 
In \cite{Ring-Wirth-2012}, superlinear convergence properties for BFGS-quasi-Newton-methods on manifolds are analysed for the case that ${\cal T}_{\eta_j}$ is
an isometry. This requirement is satisfied, e.g., if $\cal T$ and $R$
are the parallel transport and the exponential map. It is well-known (e.g.~\cite{Nocedal-Wright}) that the corresponding update of the inverse operator can be written in the form
\begin{align*}
G_{j+1}^{-1} = \left( id - \frac{s_j\otimes y_j}{g^1(y_j,s_j)} \right) \tilde{G}_j^{-1} \left(  id - \frac{y_j \otimes s_j}{g^1(y_j,s_j)} \right) + \frac{s_j\otimes s_j}{g^1(y_j,s_j)}
\end{align*}
This is the most convenient update formulation in an infinite dimensional setting.
In standard formulation, update formulas require the storage of the whole convergence history up to the current iteration. Limited memory update techniques (e.g.~\cite{Nocedal-Wright}) have been developed, in order to reduce the amount of storage. In the current situation, this can be analogously formulated in the following algorithmic way:

\begin{algorithmic}
\State $\rho_j \gets g^1(y_j,s_j)^{-1}$
\State $q \gets \grad J(c_j)$
\For{$i = j-1, \dots , j-m$}
	\State $s_i \gets {\cal T}_{q}s_i$
	\State $y_i \gets {\cal T}_{q}y_i$
	\State $\alpha_i \gets \rho_i g^1(s_i,q)$
	\State $q \gets q - \alpha_i d_i$
\EndFor
\State $z \gets \grad J(c_j)$
\State $q \gets \frac{g^1(y_{j-1},s_{j-1})}{g^1(y_{j-1},y_{j-1})} \grad J(c_j)$
\For{$i = j-m, \dots , j-1$}
	\State $\beta_i \gets \rho_i g^1(y_i,z)$
	\State $q \gets q + (\alpha_i - \beta_i) s_i$
\EndFor \\
\Return $q = G_j^{-1} \grad J(c_j)$
\end{algorithmic}
This is conceptually similar to the double loop algorithm in finite dimensional Euclidean spaces.
Yet the inner products are now given by the Sobolev metric and vector transports have to be considered.

